Hyena: Optimizing Homomorphically Encrypted Convolution for Private CNN Inference

Private inference using homomorphic encryption has gained a great attention to leverage powerful predictive models, e.g., deep convolutional neural networks (CNNs), in the area where data privacy is crucial, such as in healthcare or medical services. Processing convolution layers, however, occupies a huge portion (more than 85%) of the total latency for private CNN inference. To solve this issue, this paper presents Hyena utilizing a novel homomorphic convolution algorithm that provides speedup, communication cost, and storage saving. We first note that padded convolution provides the advantage of model storage saving, but it does not support output channel packing, thereby increasing the amount of computation and communication. We address this limitation by proposing a novel plaintext multiplication algorithm using the Walsh-Hadamard matrix. Furthermore, we propose the optimization techniques to significantly reduce the latency of the proposed convolution by selecting the optimal encryption parameters and applying lazy reduction. Overall, Hyena achieves 1.6-3.8x speedup and reduces the weight storage by 2000-8000x compared to the conventional convolution. For deep CNNs like VGG-16, ResNet-20, and MobileNetV1 on ImageNet, Hyena reduces the end-to-end latency by 1.3-2.5x, the memory usage by 2.1-7.9x and communication cost by 1.4-1.5x compared to conventional method.

==> Contents/4_Optimization.tex <==
\section{System Optimization}
\label{sec:optimization}

\ignore{
\begin{figure}[t]
\centering
%\includegraphics[width=\columnwidth]{fig/padded.png}
\includegraphics[width=\columnwidth]{Fig/op.jpg}
\caption{{(a) Permutation time vs $l_{ct}$ when $n=2048$, (b) Permutation time vs $l_{ct}$ when $n=4096$, and (c) Permutation key size and key generation time vs $l_{ct}$. The dotted line represents the approximation of execution time in a linear equation.}}
% \vspace{-1em}
\label{input}
\end{figure}
}

\subsection{Decomposition base}
Most of the time in the homomorphic rotation is spent with the costly function known as key-switching. 
It uses decomposition to divide polynomials into a number of smaller-valued coefficient polynomials, slowing the rise of noise.
If we set a $W_{dcmp}$-bit decomposition base, a single ciphertext with modulus $q$ is split into $l_{ct}=\lceil\log_{2^{W_{dcmp}}}q\rceil$ ciphertexts.
As shown in Fig.~\ref{input}, a lower decomposition base makes a single HE permutation more computationally lagging overall, operating each slice key-switching and then aggregated at the last stage.
We use a hoisting technique that divides the HE rotation process into two parts: 1) decomposing ciphertext and converting them to NTT space, and 2) key switching.
This first process is named \textbf{PermDecomp}, while the latter, an independent computation in each rotation, is named \textbf{PermAuto}.
In addition, because separate permutation keys need to be produced for each rotation, each of which is $2*n*l_{ct}*8$ B with 64-bit coefficients, key switching needs significant time and space to be performed. 
The overall key size is $2*n*l_{ct}*8*(n/2)$ B and its generation time increases linearly with $l_{ct}$ (see Fig. 6 (c)).
The latency in a single HE operation, a generation of keys, and the size of those keys are all significantly impacted by selecting a suitable $l_{ct}$.
Utilizing a large $l_{ct}$ allows the permutation key to be shared, leading to reduced key generation time and key space.
However, the operations will be slower.

\subsection{Performance modeling}
\begin{table}
\setlength{\tabcolsep}{4pt}
\centering
\caption{Runtime ($\mu$s) for HE operations used in conventional and the proposed convolution with various polynomial degree ($n$). Conventional uses the first five operations which are HRot, PermDecomp (PD.), PermAuto (PA.), HAdd, and PMult, and the proposed uses all of them with CMult+HAdd with lazy reduction (CHLR.) and reduction (R.).}
\label{operation}
{\small
%\begin{adjustbox}{width=0.45\textwidth}
\begin{tabular}{@{}C{0.8cm}@{ }C{1.4cm}@{}C{1.4cm}@{}C{1.4cm}@{}c@{ }c@{}rc@{}c}
\toprule[1.5pt]
& \multicolumn{5}{c}{\textbf{\textsl{Conventional \& Proposed}}} &
& \multicolumn{2}{c}{\textbf{\textsl{Proposed}}} \\
\cmidrule{2-6}\cmidrule{8-9}
\multirow{1}{*}{\textbf{$n$}} & \multirow{1}{*}{\textbf{HRot}} & \multirow{1}{*}{\textbf{PD.}} & \multirow{1}{*}{\textbf{PA.}} & \multirow{1}{*}{\textbf{HAdd}} & \multirow{1}{*}{\textbf{PMult}} & & \multirow{1}{*}{\textbf{{CHLR.}}} & \multirow{1}{*}{\textbf{R.}}\\
\midrule[0.2pt]
\midrule[0.2pt]
%2048 & 365 & 79+29$l_{ct}$ & 41+25$l_{ct}$ & 26+16$l_{ct}$ & 4 & 19 & 10 & 16.5 \\ [1mm]
%4096 & 770 & 161+62$l_{ct}$ & 85+55$l_{ct}$ & 56+32$l_{ct}$ & 9 & 35 & 20 & 33 \\ [0.3mm]
2048 & 85+28$l_{ct}$ & 35+23$l_{ct}$ & 27+14$l_{ct}$ & 4 & 19 
& & 10 & 16.5 \\ [1mm]
4096 & 157+64$l_{ct}$ & 74+50$l_{ct}$ & 51+30$l_{ct}$ & 9 & 35 
& & 20 & 33 \\
%\rule{0in}{2.5ex}
\bottomrule[1.5pt]
%\rule{0in}{0ex}
\end{tabular}
}
%\end{adjustbox}
\end{table}

\ignore{
\begin{algorithm}[t]
\caption{The behavior of CNN layer}
%\SetAlgoLined
\DontPrintSemicolon
\SetArgSty{textnormal}
\KwIn{$EncryptedData$}
\KwOut{$CNNResult$}

\BlankLine
\SetKwFunction{GazelleConv}{GazelleConv}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\GazelleConv{$DataCT, FilterPT$}}{
    Length of $PartialSum= $ Length of $CNNResult$\;
    %Evaluator\;
    PermDecomp($DataCT$)\;
    \For {$i \text{  in  length of  } CNNResult$} {
            \For {$j \text{  in  } f_w\cdot f_h$} {
                PermAuto($DataCT$) for $j$-step $\rightarrow RotatedCT$\;
                Multiply $RotatedCT$ and $j$-th $FilterPT$ for $i$-th $CNNResult$\;
                Add the multiplied result and $i$-th $PartialSum$\;
            }
    }
    \textbf{return} $PartialSum$\;
}

\BlankLine
\SetKwFunction{ProposedConv}{ProposedConv}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\ProposedConv{$DataCT, Hadamard Filter Scalars$}}{
    Length of $PartialSum= $ $c_n\cdot$ Length of $CNNResult$\;
    %Evaluator\;
    PermDecomp($DataCT$)\;
    \For {$i \text{  in  length of  } CNNResult$} {
            \For {$j \text{  in  } f_w\cdot f_h$} {
                PermAuto($DataCT$) for $j$-step $\rightarrow RotatedCT$\;
                \For {$k \text{  in  } c_n$} {
                    Lazy multiply $RotatedCT$ and $(j,k)$-th $filter Scalar$ for $i$-th $CNNResult$\;
                    Lazy add the above result and $(k,i)$-th $PartialSum$\;
                }
            }
    }
    \For {$i \text{  in  length of  } CNNResult$} {
        \For {$k \text{  in  } c_n$} {
            Reduce $(k,i)$-th $PartialSum$\;
            Multiply $(k,i)$-th $PartialSum$ and $k$-th $HadamardRowPT \xrightarrow{\hspace{0.2em}} (k,i)$-th $PartialSum$
        }
        Add $(k,i)$-th $PartialSum \mathrm{\,\,for} \ k$ in $c_n \rightarrow (0,i)$-th $PartialSum$
    }
    Set $i$-th $PartialSum=(0,i)$-th $PartialSum\mathrm{\,\,for} \ i $ in length of $CNNResult$\;
    \textbf{return} $PartialSum$\;
}
\BlankLine
\SetKwFunction{CNNLayer}{CNNLayer}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\CNNLayer{$EncryptedData$}}{
    \For {$i \text{  in  length of  } EncryptedData$} {
        \FuncSty{Conv}($i$-th $EncryptedData$, $Filter$)\;
        \For {$j \text{  in  length of } PartialSum$} {
            Rotate $j$-th $PartialSum$ to align the proper output channel\;
            Add the above result and $j$-th $CNNResult$\;
        }
    }
    \textbf{return} $CNNResult$\;
}
%\vspace{-1em}
\label{function}
\end{algorithm}
}
By understanding the HE operation and the mechanism of convolution, the performance of a CNN layer can be effectively modeled. 
This approach enables us to determine the optimal configuration of the network in terms of speed and memory efficiency.
Furthermore, we can balance these two factors by adjusting the $l_{ct}$ configuration accordingly, thus obtaining the most optimized network.
Table~\ref{operation} presents the execution times for each operation utilized by the two convolutions.
In the proposed scheme, lazy multiplication and addition are performed concurrently; thus, their performance is recorded as a combined measurement.
We use the results of Table~\ref{operation} for modeling.
\ignore{The behavior of the entire CNN can be described as follows: each layer in the network undergoes convolution using either Gazelle or the proposed method as outlined in Algorithm~\ref{function}.
The convolution output is then aligned through rotation to ensure consistency with the order of the output channels, resulting in the final output.
Upon receipt of encrypted data from the client, a convolution operation is performed for each input. It involves applying filters corresponding to all output channels to each input.
By performing the convolution input-by-input, it is possible to minimize the number of duplicated rotations and utilize hoisting technique.}

{Using Gazelle or the proposed convolution, the CNN layer operates according to Algorithm~\ref{function}. The client sends data ciphertexts ($EncryptedData$) which are transformed into the final output ciphertexts ($CNNResult$) using either the Gazelle or the proposed convolution (\FuncSty{GazelleConv} or \FuncSty{ProposedConv}).
The intermediate partial sums ($PartialSum$) generated after the \FuncSty{Conv} operation are rearranged through rotation to align with the order of the output channels, ultimately resulting in the final $CNNResult$.}

\ignore{Let's delve deeper into Algorithm~\ref{function}. 
As previously mentioned, this algorithm performs the convolution calculation for all outputs using the same input. 
In Gazelle, filters for all outputs for a single input must be prepared as plaintexts, with the number of plaintexts being equal to the number of output channels and the size of each filter. 
In contrast, in the proposed method, only plaintexts corresponding to the Hadamard row are used (up to two due to the maximum channel packing of two in this paper) and encoded scalar filters are needed. 
The number of additional multiplications and additions required is proportional to the number of channel packings, and the Hadamard decoding process must be performed at the end.}
{In the CNN layer, the client transmits the encrypted input data, $EncryptedData$, for all input channels.
The convolution process is then performed for each ciphertext. This is because the hoisting technique can be utilized for the same input rotation, and by creating all outputs with the use of the same rotated input $RotateCT$, we can reduce the number of rotations to a minimum.
As a result, the filter values for all output channels corresponding to each input ciphertext must be passed to \FuncSty{Conv}.
Gazelle uses the filter in plaintext ($FilterPT$), while the proposed method uses the Hadamard encoded scalar ($HadamardFilterScalars$) to generate the partial sums ($PartialSum$) corresponding to all output channels.
This results in the fastest convolution in terms of speed.}

{As mentioned earlier in the convolution process, all outputs using the common input ciphertext ($DataCT$) are generated at once. 
\FuncSty{GazelleConv} requires filters as plaintexts ($FilterPT$) as much as the length of output ciphertext (the number of output channels divided into the number of channel packing $c_n$) and filter size.
Meanwhile, in the proposed method \FuncSty{ProposedConv}, only plaintexts corresponding to the Hadamard row ($HadamardRowPT$) are used.
It is up to two as the maximum because $c_n$ is less or equal to two in this work.
The filter scalars are Hadamard-encoded ($HadamardFilterScalars$) equivalent to the length of the output ciphertext multiplied by $c_n$ and the filter size ($f_w\cdot f_h$).
In the end, additional multiplication and addition operations are necessary for the Hadamard decoding process.}

{The results of modeling the convolution layer are presented in Table~\ref{table:accuracy}.
Only Gazelle was modeled for the layers with channel packings larger than two, as the parameter optimization and latency optimization cannot be applied in such cases.
The highest error of 17\% was observed in the $(256,64,64,3)$ layer, which is due to the largest input ciphertext of 1024MB.
It leads to memory latency that cannot be accounted for in the latency calculation.
However, this error is reduced when considering the overall performance of the network, as the neural network is composed of multiple layers.
The mean absolute error (MAE) for all layers modeled with Gazelle was found to be 5.45\%. 
Moreover, this modeling still accurately reflects the overall trend of the network, making it useful in determining optimized parameters. Additionally, in determining whether Gazelle or the proposed scheme is better suited for constructing the layer, the modeled Gazelle, in less time than the actual time, is significantly larger than the proposed one modeled with an error of 2.96\%. 
It indicates that there is no problem with selecting the proposed scheme over Gazelle.}

{We modeled the key sizes and execution times of decomposition bases capable of successfully decrypting VGG-16 and ResNet-20/18 with confidence in the accuracy of the modeling. 
To determine the optimal key size and execution time, we analyzed the performance of a network comprised solely of Gazelle and a mixed network, including Gazelle and the proposed scheme.
Our findings show that the mixed networks had the lowest latency when Gazelle was used when $c_n$ was greater than two, and the proposed scheme was used when $c_n$ was less than or equal to two. 
Using this network, we swept $l_{ct}$ to obtain the orange points shown in Fig.~\ref{optimal}.
Here, the key size refers to the filter size only, with the assumption that the client is aware of the filter size of the networks used.
All networks in our work had a filter size of $3*3$, which resulted in a key size that was 128$\times$ smaller than when all permutation keys were required.
However, if the filter size is unknown, all permutation keys must be transmitted, leading to an increase in communication cost and additional storage of the keys.
In this scenario, the key size is not negligible, so finding the optimal point for key size and execution time is essential.}

{In Fig.~\ref{optimal}, three networks are displayed: (a) VGG-16, (b) ResNet-20, and (c) ResNet-18.
Blue points represent the networks consisting only of Gazelle, while orange points represent the optimized networks obtained by varying $l_{ct}$.
The red and green stars indicate the points that offer the best compromise between key size and latency.
This star point is adopted as the decomposition base set in the experiment. According to the modeling results, VGG-16 takes 1797.5 seconds on Gazelle with a key size of 8.5 MB and 752.78 seconds on the optimized one with a key size of 5.5 MB.
ResNet-20 is 144.65 seconds with 7.5 MB in Gazelle and 115.3 seconds with 5.75 MB in the optimized network.
In ResNet-18, it is 52.04 seconds with 10 MB in Gazelle and 43.93 seconds with 7.5 MB in the optimized network.}
\ignore{
\begin{table}
%\setlength\doublerulesep{.8pt}
  \centering
  \caption{Accuracy of the convolution modeling (Model.) for real runtime (seconds). Input denotes (W=H,C$_{\text{in}}$,C$_{\text{out}}$) when filter width and height are 3. MAE denotes mean absolute error.}
  \label{table:accuracy}
  %\begin{adjustbox}{width=\textwidth}
  %\begin{adjustbox}{width=10cm}
  \begin{threeparttable}
  {\small
    \begin{tabular}{@{}C{2cm}r@{}c@{ }c@{ }cr@{}c@{ }c@{ }c@{}}
    \toprule[1.5pt]
      \multicolumn{1}{c}{\multirow{2}{*}[-0.65ex]{\parbox{0.9cm}{\centering \textbf{\textit{Input}}}}} & & \multicolumn{3}{c}{\textbf{\textsl{Conventional}}} &   & \multicolumn{3}{c}{\textbf{\textsl{Proposed}}} \\
\cmidrule{3-5}\cmidrule{7-9}
{} & & \textbf{Real} & \textbf{Model.} & \textbf{Error} & & \textbf{Real} & \textbf{Model.} & \textbf{Error}\\
\midrule[0.2pt]
\midrule[0.2pt]
{(8, 256, 512)} & & 6.69 & 6.73 & \textbf{-0.67\%} & & \multicolumn{3}{c}{-} \\
{(8, 512, 512)} & & 13.56 & 13.47 & \textbf{0.7\%} & & \multicolumn{3}{c}{-} \\
{(16, 128, 256)} & & 6.03 & 6.12 & \textbf{-1.52\%} & & \multicolumn{3}{c}{-} \\
{(16, 256, 256)} & & 12.06 & 12.23 & \textbf{-1.48\%} & & \multicolumn{3}{c}{-} \\
{(16, 512, 512)} & & 43.28 & 43.97 & \textbf{-1.6\%} & & \multicolumn{3}{c}{-} \\
\cmidrule{1-1}\cmidrule{3-5}\cmidrule{7-9} 
{(32, 64, 128)} & & 2.97 & 2.83 & \textbf{4.75\%} & & 1.73 & 1.82 & \textbf{-5.62\%} \\
{(32, 128, 128)} & & 5.77 & 5.66 & \textbf{1.76\%} & & 3.48 & 3.65 & \textbf{-4.93\%} \\
{(32, 256, 512)} & & 50.52 & 47.98 & \textbf{5.02\%} & & 31.07 & 28.36 & \textbf{8.73\%} \\
{(32, 512, 512)} & & 103.04 & 95.96 & \textbf{6.87\%} & & 59.79 & 56.73 & \textbf{5.13\%} \\
%\cmidrule{1-1}\cmidrule{3-5}\cmidrule{7-9} 
{(64, 3, 64)} & & 0.19 & 0.17 & \textbf{9.34\%} & & 0.05 & 0.05 & \textbf{0.89\%} \\
{(64, 64, 64)} & & 3.97 & 3.63 & \textbf{8.55\%} & & 1.1 & 1.15 & \textbf{-4.21\%} \\
{(64, 128, 256)} & & 30.05 & 26.79 & \textbf{10.83\%} & & 8.82 & 8.25 & \textbf{6.45\%} \\
{(64, 256, 256)} & & 62.05 & 53.73 & \textbf{13.4\%} & & 17.49 & 16.51 & \textbf{5.62\%} \\
{(128, 64, 128)} & & 265.95 & 253.52 & \textbf{4.68\%} & & 86.61 & 85.95 & \textbf{0.77\%} \\
{(128, 128, 128)} & & 527.46 & 507.03 & \textbf{3.87\%} & & 174.66 & 171.9 & \textbf{1.58\%} \\
{(256, 3, 64)} & & 23.91 & 23.76 & \textbf{0.61\%} & & 8.22 & 8.05 & \textbf{2.04\%} \\
{(256, 64, 64)} & & 611.41 & 507.03 & \textbf{17.07\%} & & 177.13 & 171.89 & \textbf{2.96\%} \\
\cmidrule{1-1}\cmidrule{3-5}\cmidrule{7-9} 
{\textbf{MAE}} & & \multicolumn{3}{c}{\textbf{5.45\%}} & & \multicolumn{3}{c}{\textbf{3.76\%}} \\
    \bottomrule[1.5pt]
    \end{tabular}
    }
  \label{tab:result}%
\end{threeparttable}
  %\end{adjustbox}
\end{table}%

\begin{figure}[t]
\centering
%\includegraphics[width=\columnwidth]{fig/optimal4.png}
\includegraphics[width=\columnwidth]{Fig/optimization.jpg}
\caption{{The decision of $l_{ct}$ based on modeled execution time and key size: optimal points indicated by red star for conventional network and green star for proposed network in (a) VGG-16, (b) ResNet-20, and (c) ResNet-18.}}
% \vspace{-1em}
\label{optimal}
\end{figure}
}

==> Contents/6_Related_work.tex <==
\section{Related work}


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

